A Real-time System for Detecting Landslide Reports on Social Media using Artificial Intelligence

This paper presents an online system that leverages social media data in real time to identify landslide-related information automatically using state-of-the-art artificial intelligence techniques. The designed system can (i) reduce the information overload by eliminating duplicate and irrelevant content, (ii) identify landslide images, (iii) infer geolocation of the images, and (iv) categorize the user type (organization or person) of the account sharing the information. The system was deployed in February 2020 online at https://landslide-aidr.qcri.org/landslide_system.php to monitor live Twitter data stream and has been running continuously since then to provide time-critical information to partners such as British Geological Survey and European Mediterranean Seismological Centre. We trust this system can both contribute to harvesting of global landslide data for further research and support global landslide maps to facilitate emergency response and decision making.

==> exp_model.tex <==
\section{Model Development Experiments}
\label{sec:exp_model}

In this section, we describe the design and development of various image and text models and present experimental results. For image models, we follow the popular transfer learning approach based on convolutional neural networks (CNNs) as many studies have shown that features learned by CNNs are effectively transferable between different visual recognition tasks~\cite{JDonahue:ICML14,Sermanet:ICLR14,MOquab:CVPR14}, particularly when training samples are limited.

% TODO: on the text side, ??

\subsection{Duplicate Filtering}\label{ssec:exp_model_duplicate}
The Duplicate Filter is responsible for extracting a feature vector from a given image using a state-of-the-art deep learning model and comparing this feature vector with the feature vectors of previously seen images based on a pre-defined distance threshold $d$. For this purpose, we extract deep features from the penultimate layer of a ResNet-50 model~\cite{he2016deep} pre-trained on the Places data set~\cite{zhou2017places}, which comprises 10 million images collected for scene recognition.\footnote{The pre-trained model is available at \url{http://places2.csail.mit.edu/models_places365/resnet50_places365.pth.tar} (accessed on Jan 23, 2022).} Each feature vector has a size of 2,048. To determine the optimal distance threshold $d$, we performed experiments on a manually annotated set of 600 image pairs including 460 duplicate and 140 non-duplicate cases with varying pairwise distances. We used Euclidean distance metric (i.e., L2 norm) to measure the distance between two image feature vectors. Fig.~\ref{fig:dup_dist_distribution} shows the distribution of Euclidean distances between the image pairs for both duplicate and non-duplicate cases in our test set. Note that image pairs with a distance greater than 12.5 looked trivially distinct, and hence, we did not include them in our experiments. We then performed a grid search over a range of threshold values from 0 to 12 and measured the performance of each threshold value by computing the Matthew's Correlation Coefficient (MCC), which is regarded as a balanced measure for imbalanced classification problems~\cite{chicco2020advantages}. As depicted in Fig.~\ref{fig:dup_mcc_curve}, the optimal performance is achieved when the duplicate distance threshold is set as $d=7.1$.


\begin{figure}
    \centering
    \begin{minipage}{\columnwidth}
        \begin{subfigure}[b]{0.48\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figs/dist_distribution_grouped.png}
            \caption[Histogram of pairwise distances]{Histogram of pairwise distances}
            % {{\scriptsize Relevancy classification}}
            \label{fig:dup_dist_distribution}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.48\columnwidth}  
            \centering 
            \includegraphics[width=\columnwidth]{figs/mcc_curve.png}
            \caption[MCC vs.\ threshold]{MCC vs.\ duplicate threshold}
            % {{\scriptsize Landslide classification}}
            \label{fig:dup_mcc_curve}
        \end{subfigure}
    \end{minipage}%
    \caption[Optimal duplicate distance threshold determination. (a) Distribution of the Euclidean distances between the image pairs in the duplicate test set. (b) MCC performance as a function of distance threshold.]
    {Optimal duplicate distance threshold determination. (a) Distribution of the Euclidean distances between the image pairs in the duplicate test set. (b) MCC performance as a function of distance threshold.} 
    \label{fig:duplicate_threshold}
\end{figure}


\subsection{Junk Classification}\label{ssec:exp_model_junk}
The Junk Filter employs a CNN model to determine whether an image is relevant or not for general emergency management and response. To this end, we took a ResNet-50 model~\cite{he2016deep} pre-trained on ImageNet~\cite{ILSVRC15}, adopted its final layer to binary classification task, and fine-tuned it on a custom data set introduced by Nguyen et al.~\cite{DTNguyen:ISCRAM17}. We merged the validation set with the training set, and used the test set to evaluate the performance of the model as summarized in Table~\ref{tab:relevancy_model_data}. We used Adam optimizer~\cite{kingma2014adam} with an initial learning rate of $10^{-6}$ and configured the \texttt{ReduceLROnPlateau} scheduler to decay the learning rate by 0.1 with a patience of 50 epochs. We trained the model for a total of 200 epochs. The training process of the relevancy classification model is plotted in Fig.~\ref{fig:train_prog_relevancy} and its performance evaluation is presented in Table~\ref{tab:relevancy_model_perf}. The model achieves almost perfect performance in all measures due to the distinct features between relevant and not-relevant images in the training data set.


\begin{table}
    \caption[Details of the data set used for training the junk classification model and the performance of the trained model on the test set]{Details of the data set used for training the junk classification model and the performance of the trained model on the test set.}
    \label{tab:relevancy_model}
    \begin{subtable}{0.5\textwidth}
        \centering
        \caption{Training data set}
        \label{tab:relevancy_model_data}
        \begin{tabular}{@{}lrrr@{}}
        \toprule
        \textbf{Class} & \textbf{Train} & \textbf{Test} & \textbf{Total} \\ \midrule
        Relevant      & 2,814   & 704   & 3,518 \\
        Not-relevant  & 2,814   & 704   & 3,518 \\ \midrule
        Total         & 5,628   & 1,408 & 7,036 \\
        \bottomrule
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}{0.5\textwidth}
        \centering
        \caption{Model performance (Acc: 98.79)}
        \label{tab:relevancy_model_perf}
        \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \midrule
        Relevant       & 98.31 & 99.29 & 98.80 \\
        Not-relevant   & 99.28 & 98.30 & 98.79 \\ \midrule
        Macro avg.     & 98.80 & 98.79 & 98.79 \\
        \bottomrule
        \end{tabular}
    \end{subtable}%
\end{table}



\begin{figure}
    \centering
    \begin{minipage}{\columnwidth}
        \begin{subfigure}[b]{0.48\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figs/relevancy_training_progress.png}
            \caption[Junk classification]{Junk classification}
            % {{\scriptsize Relevancy classification}}
            \label{fig:train_prog_relevancy}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.48\columnwidth}  
            \centering 
            \includegraphics[width=\columnwidth]{figs/landslide_training_progress.png}
            \caption[Landslide classification]{Landslide classification}
            % {{\scriptsize Landslide classification}}
            \label{fig:train_prog_landslide}
        \end{subfigure}
    \end{minipage}%
    \caption[Model training progress in terms of accuracy and loss achieved on the training and validation sets]
    {Model training progress in terms of accuracy and loss achieved on the training and validation sets} 
    \label{fig:training_progress}
\end{figure}
        



\subsection{Landslide Classification}\label{ssec:exp_model_landslide}
The Landslide Detector is the most important component of the proposed system. Therefore, we performed a separate, comprehensive study to identify the optimal configuration for the landslide classification model~\cite{ofli2021landslide}. To recap, we first created a large landslide image data set labeled by landslide specialists, who are also co-authors of this paper. The data set contains 11,737 images, which are split into training, validation, and test sets as shown in Table~\ref{tab:dataset_landslide}. Then, adopting a transfer learning approach, we conducted an extensive set of experiments using various CNN architectures with different optimizers, learning rates, weight decays, and class balancing strategies. The winning model configuration is a ResNet-50 architecture trained using Adam optimizer with an initial learning rate of $10{-4}$, a weight decay of $10^{-3}$, and without a class balancing strategy. Fig.~\ref{fig:train_prog_landslide} displays the training progress of the best performing landslide classification model, which is also integrated into our system, whereas Table~\ref{tab:perf_model_landslide} summarizes the performance of the model on the test set.

\begin{table}
    \caption[Details of the data set used for training the landslide classification model and the performance of the trained model on the test set]{Details of the data set used for training the landslide classification model and the performance of the trained model on the test set.}
    \label{tab:perf_models}
    \begin{subtable}{0.5\textwidth}
        \centering
        \caption{Training data set}
        \label{tab:dataset_landslide}
        \begin{tabular}{@{}lrrrr@{}}
        \toprule
        \textbf{Class} & \textbf{Train} & \textbf{Val} & \textbf{Test} & \textbf{Total} \\ \midrule
        Landslide & 1,883 & 271 & 536 & 2,690 \\
        Not-landslide & 6,332 & 902 & 1,813 & 9,047 \\ \midrule
        Total & 8,215 & 1,173 & 2,349 & 11,737 \\
        \bottomrule
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}{0.5\textwidth}
        \centering
        \caption{Model performance (Acc: 86.97)}
        \label{tab:perf_model_landslide}
        \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \midrule
        Landslide       & 73.66 & 66.79 & 70.06 \\
        Not-landslide   & 90.45 & 92.94 & 91.68 \\ \midrule
        Macro avg.      & 82.05 & 79.87 & 80.87 \\
        \bottomrule
        \end{tabular}
    \end{subtable}%
\end{table}






% \subsection{Geolocation Inference}\label{ssec:exp_model_geolocation}
% TODO

% \subsection{User Type Classification}\label{ssec:exp_model_usertype}
% TODO


==> exp_system.tex <==
\section{System Performance Experiments}
\label{sec:exp_system}
To stress-test the system and understand its scalability, we conducted performance experiments for major critical modules. 

The experiments for image related modules were performed on a Linux machine with 256GB RAM, 2.2 GHz processor with 32 cores and two Tesla V100 GPUs with 16GB of memory. The experiment for text-related modules were performed on a Linux machine with 256GB RAM, 2.2 GHz processor with 32 cores.

\begin{figure}
    \centering
    \includegraphics[width=0.48\columnwidth]{figs/DuplicateFilterLatency.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/DuplicateFilterThroughput.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/JunkFilterLatency.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/JunkFilterThroughput.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/LandslideDetectorLatency.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/LandslideDetectorThroughput.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/GeolocationTaggerLatency.pdf}
    \hfill
    \includegraphics[width=0.48\columnwidth]{figs/GeolocationTaggerThroughput.pdf}
    \caption[Latency (left) and throughput (right) of the Junk Filter, Duplicate Filter, Landslide Detector, and Geolocation Tagger (top to bottom).]
    {Latency (left) and throughput (right) of the Junk Filter, Duplicate Filter, Landslide Detector, and Geolocation Tagger (top to bottom).} 
    \label{fig:latecy_throughput_alltogether}
\end{figure}


%Maybe mention in the start of the section
% \subsection{Hardware/System Specifications}\label{ssec:exp_sys_specs}
% TODO

\subsection{Duplicate Filter}\label{ssec:exp_sys_duplicate}
TODO

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figs/duplicate_latency.pdf}
%     \hfill
%     \includegraphics[width=0.48\columnwidth]{figs/duplicate_throughput.pdf}
%     \caption[Latency (left) and throughput (right) of the Duplicate Filter]
%     {Latency (left) and throughput (right) of the Duplicate Filter} 
%     \label{fig:latecy_throughput_duplicate}
% \end{figure}

\subsection{Junk Filter}\label{ssec:exp_sys_junk}
TODO

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figs/junk_latency.pdf}
%     \hfill
%     \includegraphics[width=0.48\columnwidth]{figs/junk_throughput.pdf}
%     \caption[Latency (left) and throughput (right) of the Junk Filter]
%     {Latency (left) and throughput (right) of the Junk Filter} 
%     \label{fig:latecy_throughput_junk}
% \end{figure}






\subsection{Landslide Detector}\label{ssec:exp_sys_landslide}
TODO

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figs/landslide_latency.pdf}
%     \hfill
%     \includegraphics[width=0.48\columnwidth]{figs/landslide_throughput.pdf}
%     \caption[Latency (left) and throughput (right) of the Landslide Detector]
%     {Latency (left) and throughput (right) of the Landslide Detector} 
%     \label{fig:latecy_throughput_landslide}
% \end{figure}


\subsection{Geolocation Tagger}\label{ssec:exp_sys_geolocation}
TODO

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figs/geotagger_latency.pdf}
%     \hfill
%     \includegraphics[width=0.48\columnwidth]{figs/geotagger_throughput.pdf}
%     \caption[Latency (left) and throughput (right) of the Geolocation Tagger]
%     {Latency (left) and throughput (right) of the Geolocation Tagger} 
%     \label{fig:latecy_throughput_geolocation}
% \end{figure}

